NISPA: Neuro-Inspired Stability-Plasticity Adaptation for Continual Learning in Sparse Networks

The goal of continual learning (CL) is to learn different tasks over time. The main desiderata associated with CL are to maintain performance on older tasks, leverage the latter to improve learning of future tasks, and to introduce minimal overhead in the training process (for instance, to not require a growing model or retraining). We propose the Neuro-Inspired Stability-Plasticity Adaptation (NISPA) architecture that addresses these desiderata through a sparse neural network with fixed density. NISPA forms stable paths to preserve learned knowledge from older tasks. Also, NISPA uses connection rewiring to create new plastic paths that reuse existing knowledge on novel tasks. Our extensive evaluation on EMNIST, FashionMNIST, CIFAR10, and CIFAR100 datasets shows that NISPA significantly outperforms representative state-of-the-art continual learning baselines, and it uses up to ten times fewer learnable parameters compared to baselines. We also make the case that sparsity is an essential ingredient for continual learning. The NISPA code is available at https://github.com/BurakGurbuz97/NISPA.

==> content/main/3_nispa.tex <==
\section{NISPA description}
\begin{figure*}[ht]
\begin{center}
\centerline{\includegraphics[width=\textwidth]{figures/main_figure.png}}
\caption{The training for each task is divided into ``phases`` ($e$ epochs each). Between successive tasks, we select candidate stable units, and the rewiring process takes place. On the task boundaries, survived candidate units are promoted to old stable units. Finally, we freeze all connections between old stable units and reinitialize the remaining connections.}
\label{fig:main_figure}
\end{center}
\vskip -0.4in
\end{figure*}

%In brief, NISPA splits the network into stable and plastic units. We preserve the functionality of stable units so that the network retains learned knowledge and mitigates CF. Additionally, rewiring creates novel paths and enables forward transfer learning. 

\textbf{Figure}~\ref{fig:main_figure} illustrates the key ideas in NISPA, 
while \textbf{Algorithm}~\ref{alg:method} (see Appendix) presents the complete method. 
The training for each task is divided into ``phases`` ($e$ epochs each).  After each phase, we select {\em candidate stable units} $S_c^l$ (Section \ref{selection}). This selection step is followed by {\em connection rewiring} (Section \ref{rewiring}) at each phase. This selection and rewiring cycle is repeated for several phases until the {\em stopping criterion} is met (Section \ref{stopping}). Once a task ends, we freeze the incoming connections of all stable units (Section \ref{stabilizing}). 


\subsection{Notation and Problem Formulation}
In most of the paper we consider task incremental learning, with a sequence of $T$ tasks. For each task $t$ we have a training dataset $D_t$ and a validation dataset $V_t$. Task identifiers are available during training and testing. The layer $l \in \left\{ 1, \dots, L \right\}$ has $N_l$ nodes and let $n_i^l \in  \left\{ 1, \dots, N_l \right\}$ be the $i$-th unit in that layer. Moreover, let $\theta_{i, j}^l$ denote the  $j$-th incoming connection of $n_i^l$ from $n_j^{l - 1}$. We denote the activation of unit $n_i^l$ as $a_{n_i^l}(x)$ and the total activation of layer $l$ as $a_{l}(x)$, where $x$ is the input that generates these activations. 
The activation function of all units, except the outputs, is ReLU.

For convolutional neural networks (CNNs), a ``unit'' is replaced by a 3D convolution filter. Likewise, a ``connection'' is replaced by a 2D kernel. 
\subsection{Stabilizing a Plastic Unit} \label{stabilizing}
The activation of unit $n_i^l$ is determined by its parent units' activations and the weight of incoming connections from those parents. So, any weight updates during training alter unit  $n_i^l$ in two ways: first, directly changing the weights of incoming connections to the  unit. Second, indirectly, by changing the weights of incoming connections to the unit's ancestor units, i.e., units in any path from the inputs to $n_i^l$. NISPA ensures that  stable units receive input only from other stable units. This is achieved by ``freezing'' connections between stable units at the task boundaries, i.e., not allowing the corresponding weights to change after that point.


\subsection{Selecting Candidate Stable Units} \label{selection}
At any given time, the units $U^l$ of layer $l$ are partitioned into two disjoint sets $S^l$ and $P^l$, namely stable and plastic units respectively. $S^l$  is further divided into two disjoint sets $S^l \equiv S_o^l \cup S_c^l $ where $S_o^l$ refers to ``old'' stable units, and $S_c^l$ ``candidate'' stable units. While learning task $t$, NISPA periodically transitions some plastic units from $P^l$ into the set of candidate stable units $S_c^l$.
At the end of that task's training, the members of $S_c^l$ are moved into $S_o^l$.

Suppose we start with 
the sets $P^l$ and $S_o^l$ we inherited from the previous task -- if there is no previous task, all units are plastic. First, we compute the total activation at each layer across all training examples for that task, as follows: 
\begin{equation}
    A_l =  \sum_{x \in D_t} a_l(x) =  \sum_{x \in D_t} \sum_{i = 1}^{N_l}   a_{n_i^l}(x)
\end{equation}
Next, for each layer we select the candidate stable units $S_c^l$ as follows:
\begin{equation}
\underset{S_c^l \subseteq P^l}{\min} \left| S_c^l \right| \; \text{subject to} \; \sum_{x \in D_t}   \sum_{n_i^l \in S_c^l \cup S_o^l} a_{n_i^l}(x)  \geq \tau  A_l 
\end{equation}
So, the aim is to compute the smallest set of units $S_c^l \subseteq P^l$ that we need to add to $S_o^l$ to capture at least a fraction $\tau$  of the total activation of layer $l$ (the selection of  $\tau$ is discussed later in this section). 
Then we remove those elements of $S_c^l$ from $P^l$.

The previous optimization problem is solved heuristically, as follows. We start with $S_c^l \equiv \emptyset$. Then we add plastic units with the largest total activation one by one into $S_c^l$ until the $\tau$ criterion is satisfied. If $S_o^l$ already captures at least $\tau$ fraction of the overall layer activation, the algorithm does not select any candidate stable units and $S_c^l$ is empty. Note that the selection process is performed in parallel at each layer. 
The  input and output layers do not participate in this process because they are considered stable.

The rationale of this approach is that units in $S_c^l$ are highly active while learning task $t$. So, to avoid forgetting that task in the future, we stabilize these units by disabling any gradient updates in their input paths. 


\textbf{Determining $\tau$: }In the early phases of a task's training, the activations can vary erratically. So, it is better to start with a larger $\tau$, meaning that more candidate stable units $S_c^l$ will be selected.  As the training proceeds, the network becomes more competent in that task, and we can further restrict the selection of candidate stable units. 

This intuition suggests a gradual reduction of $\tau$, starting with $\tau_1 = 1$ in the first phase, and decreasing $\tau$ in step sizes that increase with every phase. To do so we use the following cosine annealing schedule:
 \begin{equation}
    \tau_p =\frac{1}{2} \left ( 1 + \cos \left ( \frac{p \times \pi}{k} \right ) \right )
\end{equation},  where $p$ is the phase number and $k$ is a hyperparameter that determines the shape of the function.



\begin{figure}[ht]
\begin{center}
\centerline{\includegraphics[width=\columnwidth]{figures/activation_analysis.png}}
\caption{A and B show the activation distributions in a sparse (90\% pruned) two-layer multilayer perceptron after training on MNIST -- both distributions are highly skewed. C demonstrates that skewness does not change much during training. D shows that the removal of highly active units hurts the performance of the model much more than the removal of other units.}
\label{fig:activation_analysis}
\end{center}
\end{figure}



\textbf{Skewness of activations:} 
One may ask whether too many units will be selected as stable, not leaving enough plastic units for subsequent tasks.
Prior work  has observed that using ReLUs leads to a per-layer unit activation distribution that is highly skewed across different network architectures and datasets \cite{sparse_sensitivity, Trimming, DMA, Georgios2018} -- the main reason is that a ReLU maps all negative pre-activations to zero. As a result, the activation of most units is almost zero, while only few units show a large activation. \textbf{Figure}~\ref{fig:activation_analysis}-A,B show an example of this phenomenon on an MNIST classification task. Recall that, given samples $\left\{ x_1, \dots, x_n \right\}$ and their mean $\bar{x}$, the sample skewness is defined as:
\begin{equation}
    g_1 = \frac{ \frac{1}{n} \sum_{i = 1}^{n} (x_i  - \bar{x})^3}{\left [ \frac{1}{n} \sum_{i = 1}^{n} (x_i  - \bar{x})^2 \right ]^{1.5}}
\end{equation}
\textbf{Figure}~\ref{fig:activation_analysis}-C shows how the skewness of the activation distribution (one per layer) is high even at the first epoch,  and it remains high throughout the training period. 

This is an important point for NISPA because it suggests that we can satisfy the $\tau A_{l}$ constraint by selecting only few units from the right tail of the distribution (i.e., the most active units). This ensures that there are many  units will remain plastic for learning future tasks.


\textbf{Activation as a measure of importance:} 
Another concern may be whether the total activation of a unit is a valid indicator of its contribution to learning a task.
Activations are often used to determine which units are more important for a given task in problems such as CL \cite{AGS-CL, neural_pruning}, network pruning \cite{sparse_sensitivity, Trimming, DMA}, and  network interpretation \cite{erhan2009, zeiler2013}. There are several empirical results that support this choice, such as the observation  that removing the most active units degrades the performance much more than removing the same number of randomly chosen units \cite{AGS-CL}. Similar results for the MNIST classification task are shown in \textbf{Figure}~\ref{fig:activation_analysis}-D, highlighting the strong correlation between a unit's activation and its importance for a given task.


\subsection{Connection Rewiring} \label{rewiring}
NISPA leverages connection rewiring for two reasons: mitigate forgetting and create novel pathways for forward transfer. Rewiring follows the selection of candidate stable units $S_c^l$ at the end of each phase, and it consists of (1) dropping and (2) growing connections, as described next. 

(1) We remove connections from plastic units to stable units. So, future changes in a plastic unit's functionality are not propagated to  stable units. More formally, given $S_o^l$, $P^l$, and $S_c^l$,  all connections $\theta_{i, j}^l$ where $n_i^l \in S_o^l \cup S_c^l$ and $n_j^{l - 1} \in P^{l-1}$ are dropped. 

(2) Dropping some connections from a layer $l$ is followed by growing the same number of new connections in layer $l$.
In other words, NISPA maintains the per-layer network density. The new connections are selected randomly as long as they do not form new inputs to stable units (i.e., $\theta_{i, j}^l$ where $n_i^l \in P^l$ and $n_j^{l - 1} \in P^{l-1} \cup S^{l - 1}$). This guarantees that the growing mechanism will not disrupt representations learned by stable units. 

The weight of new connections is initialized based on existing weights, as follows. Let  $\mu_l$ be the mean and $\sigma_l$ the standard deviation of the existing weights at layer $l$. We sample a new weight as $\theta^l \sim \mathcal{N}_l(\mu_l, \sigma_l)$. 

NISPA only grows connections between plastic units (type-1) or from stable units to plastic units (type-2). Type-1 and type-2 connections serve different purposes. Type-1 connections may enable learning new representations for future tasks. In contrast, type-2 connections promote forward transfer, as plastic units can utilize learned and stable representations.  Depending on the similarities across tasks and the layer at which the connections are added, type-1 could be more or less valuable than type-2. We have not optimized the choice between the two types.

%\textcolor{blue}{In contrast to NISPA, regularization approaches address only the first source of interference by penalizing change in connections, overlooking the latter. So, a slight alteration in the initial layers accumulated throughout the network, creating a cascade effect that significantly alters units at the top layers. We note that this difference makes NISPA more resistant to forgetting.}
 

%  \begin{algorithm}[tb]
%   \caption{\textcolor{blue}{NISPA on task $t$ (repeated for every task)}}
%   \label{alg:method}
% \begin{algorithmic}[1]
%   \REQUIRE $S_{o}$, $e$, $a_{f}$, $k$, $M$ \COMMENT{$M$ is the model}
%   \STATE $a_{max} \gets 0$, $\tau \gets 1$, $p \gets 1$  \COMMENT{$p$ is the phase index}
%   \LOOP
%      \STATE $M \gets \textbf{Train}(M, e, D_t)$ \COMMENT{use training set $D_t$}
%      \STATE $\text{CacheM}[p] \gets M$ \COMMENT{Store the model}
%      \STATE $a \gets \textbf{Validate}(M, V_t)$ \COMMENT{use validation set $V_t$}
%      \STATE $a_{max} \gets \max(a_{max}, a)$
%      \IF {$a_{max} - a_{f} \leq a $}
%          \STATE $\tau \gets \frac{1}{2} \left ( 1 + \cos \left ( \frac{p \times \pi}{k} \right ) \right ) $
%          \STATE $S \gets \textbf{SelectCandidates}(M, S_o, \tau)$
%          \STATE $\text{CacheS}[p] \gets S$ \COMMENT{Store set of stable units}
%          \STATE{\# Drop connections from $P^l$ to $S^{l+1}$}
%          \STATE $M \gets \textbf{Drop}(M, S)$ 
%          \STATE{\# Randomly grow connections from $U^l$ to $P^{l+1}$}
%          \STATE $M \gets \textbf{Grow}(M, S)$ 
%          \STATE $p \gets p + 1$ \COMMENT{Increase the phase index}
%      \ELSE
%         \STATE $M \gets \text{CacheM}[p - 1]$ \COMMENT{Restore saved $M$}
%         \STATE $S_o \gets \text{CacheS}[p - 2]$ \COMMENT{Restore saved $S$}
%         \STATE{\# Freeze connections from $S^l$ to $S_o^{l+1}$}
%         \STATE $M \gets \textbf{Freeze}(M, S_o)$ 
%         \STATE{\# Reinitialize connections from $U^l$ to $P^{l+1}$}
%         \STATE $M \gets \textbf{Reinit}(M, S_o)$ 
%         \STATE \textbf{return} $M$, $S_o$ \COMMENT{Start task $t+1$}
%      \ENDIF
%   \ENDLOOP
% \end{algorithmic}
% \end{algorithm}


\textbf{Stopping criterion: } We do not fix the number of phases. Instead, we track the highest  accuracy  achieved so far on the validation dataset $V_t$.  At the end of a phase, if the new accuracy is  worse than the best accuracy (the difference is more than $a_f$), we stop training and revert the model to the end of the previous phase, perform freezing and pass the stable units to the next task. In other words, we perform early stopping at the level of phases instead of epochs.  

Note that a task ends with a last sequence of $e$ epochs. This allows the network to recover from any performance loss due to the last rewiring process.

We observed that plastic units start with a bias from the last tasks, which hinders learning a new task. Motivated by this observation, we re-initialize the weights of all non-frozen connections before beginning a new task.




==> review/response.tex <==
documentclass{article}

% Please use the following line and do not change the style file.
\usepackage{icml2022_author_response}

% Recommended, but optional, packages for figures and better typesetting:
\usepackage{microtype}
\usepackage{graphicx}
\usepackage{subfigure}
\usepackage{hyperref}       % hyperlinks
\usepackage{booktabs} % for professional tables
\usepackage{amsfonts}       % blackboard math symbols
\usepackage{nicefrac}       % compact symbols for 1/2, etc.
\usepackage{amsmath}
\usepackage{lipsum}

\begin{document}
We are grateful to the reviewers for their time and
constructive comments. We will correct any grammatical issues the reviewers identified. Furthermore, we will  update the Algorithm-1 description to remove any ambiguity and add standard deviations in all relevant plots.

\subsection*{Reviewer 2}
\textbf{Choice of Architecture: } DNN architectures are based on [Zenke2017]. However, our tasks are more challenging compared to  [Zenke2017]. For example, instead of MNIST, we use a combination of EMNIST and FMNIST, or we use all CIFAR100 classes instead of the first 50. Therefore, we tweaked the original architectures to give all baselines extra learning capacity. However, we note that these slight changes do not affect the conclusions.

\textbf{Choice of Baselines: } NISPA does not rely on model expansion or rehearsal. Consequently, only regularization-based methods and few isolation approaches share the same constraints. So, we picked the three well-known regularization methods (EWC, SI, and MAS) and an isolation approach (CLNP) most similar to NISPA as our benchmarks.  

\emph{Please see the Reviewer 6 section for our response regarding class-incremental scenario experiments.}

\subsection*{Reviewer 5}
\textbf{Clarification of the Algorithm: } Algorithm-1  shows the steps for a \emph{single task}, and $t$ denotes the \emph{phase index} as commented. So, one loop iteration shows the steps for a single phase, not a task. We understand $t$ misleads the reader as $t$ commonly refers to the task index. We will update the Algorithm-1 description and use more precise notation.

\textbf{Presentation Details: } We will improve the presentation of figures and tables based on the feedback of the reviewer.

\subsection*{Reviewer 6}
\textbf{Need of Task Labels: }  We agree that requiring task labels during testing limits NISPA's applicability to more realistic scenarios. This limitation is shared by almost all methods ([van de Ven2019]) that do not rely on rehearsal. However, NISPA only requires task labels to pick the correct classification head -- all other layers are agnostic to task labels. In other words, task information is only used between the penultimate and classification layers. This is significantly different from task-incremental learners, which rely on task information throughout the architecture (e.g., [Rusu2016]). Therefore, the main ideas behind NISPA are not specific to task-incremental learning, and NISPA would also work in a class-incremental scenario with an improved classification layer. We are already working on an extension to address this limitation, and we are committed to adding these results in the final paper.

\textbf{Comparison with Rehearsal Methods: } Prior work (e.g., [Prabhu2020]) showed that even naive rehearsal approaches outperform SOTA methods that do not use rehearsal in class-incremental learning. So, for fair evaluation, we compare NISPA with methods that make the same assumptions -- task labels are given and no access to examples of earlier tasks. 

Our ongoing work to make NISPA a class incremental learner relies on a small experience buffer. So, we aim to have a separate evaluation that compares this version of NISPA with rehearsal methods in the class-incremental scenario in the final paper. We think this evaluation will provide more insights than comparing task-incremental NISPA with class-incremental rehearsal methods.

\textbf{Clarity Regarding Scenario: } We agree with the reviewer that a clear statement  regarding the learning scenario should be mentioned earlier in the text. We will clearly state in the abstract and introduction that the original version of NISPA requires task labels during testing to avoid misconceptions.

\textbf{Rehearsal in the Brain: } We agree that the brain employs some form of rehearsal through memory consolidation processes. Our comment regarding the absence of rehearsal concerns storing "raw" examples (e.g., pixel-level). We will clarify that paragraph to avoid ambiguity.

\subsection*{Reviewer 7}
\textbf{Comparison of Number of Parameters: } Details for the number of parameters are given in the Experimental Results section. (line 300) \emph{"We use MLP with 80\% sparsity and CNN with 90\% sparsity on all experiments."}  (line 282) \emph{"EWC, SI, MAS, and CLNP use dense networks, giving them five to ten times more learnable parameters compared to NISPA."} We will include quantitative comparisons in the figures to support our claim more precisely.

\textbf{EMNIST + FMNIST results: } Note that CLNP has more parameters since it starts with a dense network, while NISPA has a fixed sparsity of 80\%. CLNP drops connections between tasks, but it never reaches the sparsity level of NISPA. For example, in our experiments CLNP has a sparsity of 23.91\% and 26.93\% before starting task-4 and task-5, respectively. So, the slightly better performance of CLNP can be attributed to the extra parameters. This does not necessarily mean that CLNP leverages the previous knowledge more effectively or better generalizes to an unrelated dataset.

\textbf{Unfreezing Mechanism: } As highlighted in the conclusion section, we agree with the reviewer that future work on unfreezing mechanism is needed to let NISPA continue learning even on very long task sequences.

\textbf{References}

[Zenke2017]: arxiv.org/abs/1703.04200

[van de Ven2019]: arxiv.org/abs/1904.07734

[Rusu2016]: arxiv.org/abs/1606.04671

[Prabhu2020]: robots.ox.ac.uk/~tvg/publications/2020/gdumb.pdf





\end{document}

